Enabling Kernel Bypass Networking on gem5

Full-system simulation of computer systems is critical to capture the complex interplay between various hardware and software components in future systems. Modeling the network subsystem is indispensable to the fidelity of the full-system simulation due to the increasing importance of scale-out systems. The network software stack has undergone major changes over the last decade, and kernel-bypass networking stacks and data-plane networks are rapidly replacing the conventional kernel network stack. Nevertheless, the current state-of-the-art architectural simulators still use kernel networking which precludes realistic network application scenarios. In this work, we enable kernel bypass networking stack on gem5, the state-of-the-art full-system architectural simulator. We extend gem5's NIC hardware model and device driver to enable the support for userspace device drivers to run the DPDK framework. We also implement a network load generator hardware model in gem5 to generate various traffic patterns and perform per-packet timestamp and latency measurements without introducing packet loss. Our experimental results show that DPDK's simulated network bandwidth scales with the number of cores and NIC ports. As two use cases, we analyze the sensitivity of (1) network performance to several microarchitectural parameters, and (2) direct cache access (DCA) technology to DPDK burst size.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> code-changes/byte-offset-write-PCI-COMMAND.tex <==
FILE :: gem5/src/dev/pci/device.cc

Tick
PciDevice::writeConfig(PacketPtr pkt)
{
    int offset = pkt->getAddr() & PCI_CONFIG_SIZE;

    /* No effect if we write to config space that is not implemented*/
    if (offset >= PCI_DEVICE_SPECIFIC &&
        offset < PCI_CONFIG_SIZE) {
        warn_once("Device specific PCI config space "
                  "not implemented for %s!\n", this->name());
        switch (pkt->getSize()) {
            case sizeof(uint8_t):
            case sizeof(uint16_t):
            case sizeof(uint32_t):
                break;
            default:
                panic("invalid access size(?) for PCI configspace!\n");
        }
    } else if (offset > PCI_CONFIG_SIZE) {
        panic("Out-of-range access to PCI config space!\n");
    }

    switch (pkt->getSize()) {
      uint8_t low_command_bits;
      case sizeof(uint8_t):
        switch (offset) {
          case PCI0_INTERRUPT_LINE:
            config.interruptLine = pkt->getLE<uint8_t>();
            break;
          case PCI_CACHE_LINE_SIZE:
            config.cacheLineSize = pkt->getLE<uint8_t>();
            break;
          case PCI_LATENCY_TIMER:
            config.latencyTimer = pkt->getLE<uint8_t>();
            break;
          // ADDITION Handle Misalgined commmand reg write
          case 0x5:
            low_command_bits = config.command & 0xFF;
            config.command = (pkt->getLE<uint8_t>() << 8) | low_command_bits;
            break;
          /* Do nothing for these read-only registers */
          case PCI0_INTERRUPT_PIN:
          case PCI0_MINIMUM_GRANT:
          case PCI0_MAXIMUM_LATENCY:
          case PCI_CLASS_CODE:
          case PCI_REVISION_ID:
            break;
          default:
            panic("writing to a read only register  %#x\n", offset);
        }
        DPRINTF(PciDevice,
            "writeConfig: dev %#x func %#x reg %#x 1 bytes: data = %#x\n",
            _busAddr.dev, _busAddr.func, offset,
            (uint32_t)pkt->getLE<uint8_t>());
        break;
      case sizeof(uint16_t):
        switch (offset) {
          case PCI_COMMAND:
            config.command = pkt->getLE<uint16_t>();
            // IO or memory space may have been enabled/disabled.
            pioPort.sendRangeChange();
            break;
          case PCI_STATUS:
            config.status = pkt->getLE<uint16_t>();
            break;
          case PCI_CACHE_LINE_SIZE:
            config.cacheLineSize = pkt->getLE<uint8_t>();
            break;
          default:
            panic("writing to a read only register");
        }
        DPRINTF(PciDevice,
            "writeConfig: dev %#x func %#x reg %#x 2 bytes: data = %#x\n",
            _busAddr.dev, _busAddr.func, offset,
            (uint32_t)pkt->getLE<uint16_t>());
        break;
      case sizeof(uint32_t):
        switch (offset) {
          case PCI0_BASE_ADDR0:
          case PCI0_BASE_ADDR1:
          case PCI0_BASE_ADDR2:
          case PCI0_BASE_ADDR3:
          case PCI0_BASE_ADDR4:
          case PCI0_BASE_ADDR5:
            {
                int num = BAR_NUMBER(offset);
                auto *bar = BARs[num];
                config.baseAddr[num] =
                    htole(bar->write(hostInterface, pkt->getLE<uint32_t>()));
                pioPort.sendRangeChange();
            }
            break;

          case PCI0_ROM_BASE_ADDR:
            if (letoh(pkt->getLE<uint32_t>()) == 0xfffffffe)
                config.expansionROM = htole((uint32_t)0xffffffff);
            else
                config.expansionROM = pkt->getLE<uint32_t>();
            break;

          case PCI_COMMAND:
            // This could also clear some of the error bits in the Status
            // register. However they should never get set, so lets ignore
            // it for now
            config.command = pkt->getLE<uint32_t>();
            // IO or memory space may have been enabled/disabled.
            pioPort.sendRangeChange();
            break;

          default:
            DPRINTF(PciDevice, "Writing to a read only register");
        }
        DPRINTF(PciDevice,
            "writeConfig: dev %#x func %#x reg %#x 4 bytes: data = %#x\n",
            _busAddr.dev, _busAddr.func, offset,
            (uint32_t)pkt->getLE<uint32_t>());
        break;
      default:
        panic("invalid access size(?) for PCI configspace!\n");
    }
    pkt->makeAtomicResponse();
    return configDelay;
}


==> figures/float-sensitivity.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figures/arch-sensitivity.pdf}
\vspace{-5pt}
\caption{Sensitivity of \fwd to architectural parameters.}
\vspace{-20pt}
\label{fig:sensitivity}
\end{center}
\end{figure}


==> figures/float-validation.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figures/validation.pdf}
\vspace{-5pt}
\caption{Maximum sustainable network bandwidth of \fwd running on gem5 for different packet sizes. }
%Single NIC bandwidth comparison between real hardware and simulated system.}
\vspace{-20pt}
\label{fig:validation}
\end{center}
\end{figure}
